MixPE: Quantization and Hardware Co-design for Efficient LLM Inference

Transformer-based large language models (LLMs) have achieved remarkable success as model sizes continue to grow, yet their deployment remains challenging due to significant computational and memory demands. Quantization has emerged as a promising solution, and state-of-the-art quantization algorithms for LLMs introduce the need for mixed-precision matrix multiplication (mpGEMM), where lower-precision weights are multiplied with higher-precision activations. Despite its benefits, current hardware accelerators such as GPUs and TPUs lack native support for efficient mpGEMM, leading to inefficient dequantization operations in the main sequential loop. To address this limitation, we introduce MixPE, a specialized mixed-precision processing element designed for efficient low-bit quantization in LLM inference. MixPE leverages two key innovations to minimize dequantization overhead and unlock the full potential of low-bit quantization. First, recognizing that scale and zero point are shared within each quantization group, we propose performing dequantization after per-group mpGEMM, significantly reducing dequantization overhead. Second, instead of relying on conventional multipliers, MixPE utilizes efficient shift\&add operations for multiplication, optimizing both computation and energy efficiency. Our experimental results demonstrate that MixPE surpasses the state-of-the-art quantization accelerators by $2.6\times$ speedup and $1.4\times$ energy reduction.

==> figs/gemm <==
<mxfile host="Electron" agent="Mozilla/5.0 (Windows NT 10.0; Win64; x64) AppleWebKit/537.36 (KHTML, like Gecko) draw.io/24.7.17 Chrome/128.0.6613.36 Electron/32.0.1 Safari/537.36" version="24.7.17">
  <diagram name="第 1 页" id="w3LjGgpXsp95ZFat9aOV">
    <mxGraphModel dx="1036" dy="614" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="827" pageHeight="1169" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="yMBw17B98Hdd5w8U56Xl-112" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=none;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="780" y="340" width="110" height="190" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-101" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=none;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="625" y="280" width="123" height="250" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-81" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=none;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="473" y="320" width="112" height="210" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-9" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="200" y="440" width="120" height="90" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-1" value="" style="rounded=0;whiteSpace=wrap;html=1;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry width="120" height="90" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-4" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-9" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="30" as="sourcePoint" />
            <mxPoint x="120" y="30" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-5" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-9" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="60" as="sourcePoint" />
            <mxPoint x="120" y="60" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-6" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-9" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="30" as="sourcePoint" />
            <mxPoint x="30" y="90" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-7" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-9" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="59.5" as="sourcePoint" />
            <mxPoint x="59.5" y="90" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-8" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-9" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="90" as="sourcePoint" />
            <mxPoint x="90" y="90" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-37" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-38" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry x="30" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-40" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry x="60" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-43" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry x="90" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-35" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=none;dashed=1;strokeColor=#1A1A1A;strokeWidth=1;" parent="yMBw17B98Hdd5w8U56Xl-9" vertex="1">
          <mxGeometry x="-4" y="-4" width="68" height="38" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-23" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="340" y="302" width="90" height="120" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-17" value="" style="rounded=0;whiteSpace=wrap;html=1;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry width="90" height="120" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-18" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-23" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="30" as="sourcePoint" />
            <mxPoint x="30" y="120" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-19" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-23" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="60" as="sourcePoint" />
            <mxPoint x="60" y="120" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-20" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-23" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="30" as="sourcePoint" />
            <mxPoint x="90" y="30" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-21" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-23" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="59.5" as="sourcePoint" />
            <mxPoint x="90" y="59.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-22" value="" style="endArrow=none;html=1;rounded=0;" parent="yMBw17B98Hdd5w8U56Xl-23" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="90" as="sourcePoint" />
            <mxPoint x="90" y="90" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-34" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E6D0DE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-33" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E6D0DE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry y="30" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-39" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCE9F;strokeColor=#d79b00;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry y="60" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-42" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCE9F;strokeColor=#d79b00;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry y="90" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-45" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=none;dashed=1;strokeColor=#1A1A1A;strokeWidth=1;direction=south;" parent="yMBw17B98Hdd5w8U56Xl-23" vertex="1">
          <mxGeometry x="-4" y="56" width="38" height="68" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-24" value="&lt;font style=&quot;font-size: 24px;&quot;&gt;m&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="150" y="470" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-25" value="&lt;font style=&quot;font-size: 24px;&quot;&gt;k&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="250" y="407" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-26" value="&lt;font style=&quot;font-size: 24px;&quot;&gt;k&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="290" y="320" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-27" value="&lt;font style=&quot;font-size: 24px;&quot;&gt;n&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="355" y="270" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-28" value="" style="rounded=0;whiteSpace=wrap;html=1;" parent="1" vertex="1">
          <mxGeometry x="340" y="440" width="90" height="90" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-29" value="" style="endArrow=none;html=1;rounded=0;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="340" y="470" as="sourcePoint" />
            <mxPoint x="430" y="470" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-30" value="" style="endArrow=none;html=1;rounded=0;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="340" y="500" as="sourcePoint" />
            <mxPoint x="430" y="500" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-31" value="" style="endArrow=none;html=1;rounded=0;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="370" y="440" as="sourcePoint" />
            <mxPoint x="370" y="530" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-32" value="" style="endArrow=none;html=1;rounded=0;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="400" y="440" as="sourcePoint" />
            <mxPoint x="400" y="530" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-36" value="&lt;font style=&quot;font-size: 15px;&quot;&gt;Group 1&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="200" y="410" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-41" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCCCC;strokeColor=#a31f35;" parent="1" vertex="1">
          <mxGeometry x="340" y="440" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-46" value="&lt;font style=&quot;font-size: 15px;&quot;&gt;Group 2&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;direction=north;flipV=0;flipH=0;horizontal=0;" parent="1" vertex="1">
          <mxGeometry x="310" y="362" width="30" height="60" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-49" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;1. Dequant&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=13;" parent="1" vertex="1">
          <mxGeometry x="477" y="320" width="92" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-51" value="&lt;span style=&quot;color: rgba(0, 0, 0, 0); font-family: monospace; font-size: 0px; text-align: start; text-wrap: nowrap;&quot;&gt;%3CmxGraphModel%3E%3Croot%3E%3CmxCell%20id%3D%220%22%2F%3E%3CmxCell%20id%3D%221%22%20parent%3D%220%22%2F%3E%3CmxCell%20id%3D%222%22%20value%3D%22%22%20style%3D%22rounded%3D0%3BwhiteSpace%3Dwrap%3Bhtml%3D1%3BfillColor%3D%23E6D0DE%3BstrokeColor%3D%23B5739D%3B%22%20vertex%3D%221%22%20parent%3D%221%22%3E%3CmxGeometry%20x%3D%22580%22%20y%3D%22370%22%20width%3D%2230%22%20height%3D%2230%22%20as%3D%22geometry%22%2F%3E%3C%2FmxCell%3E%3C%2Froot%3E%3C%2FmxGraphModel%3E&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E6D0DE;strokeColor=#B5739D;" parent="1" vertex="1">
          <mxGeometry x="485" y="388" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-59" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="638" y="302" width="100" height="100" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-54" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-59" vertex="1">
          <mxGeometry y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-55" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-59" vertex="1">
          <mxGeometry x="30" y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-56" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-59" vertex="1">
          <mxGeometry x="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-57" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-59" vertex="1">
          <mxGeometry x="70" y="30" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-58" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="yMBw17B98Hdd5w8U56Xl-59" vertex="1">
          <mxGeometry x="70" y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-69" value="&lt;span style=&quot;color: rgba(0, 0, 0, 0); font-family: monospace; font-size: 0px; text-align: start; text-wrap: nowrap;&quot;&gt;%3CmxGraphModel%3E%3Croot%3E%3CmxCell%20id%3D%220%22%2F%3E%3CmxCell%20id%3D%221%22%20parent%3D%220%22%2F%3E%3CmxCell%20id%3D%222%22%20value%3D%22%22%20style%3D%22rounded%3D0%3BwhiteSpace%3Dwrap%3Bhtml%3D1%3BfillColor%3D%23E6D0DE%3BstrokeColor%3D%23B5739D%3B%22%20vertex%3D%221%22%20parent%3D%221%22%3E%3CmxGeometry%20x%3D%22580%22%20y%3D%22370%22%20width%3D%2230%22%20height%3D%2230%22%20as%3D%22geometry%22%2F%3E%3C%2FmxCell%3E%3C%2Froot%3E%3C%2FmxGraphModel%3E&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E6D0DE;strokeColor=#B5739D;" parent="1" vertex="1">
          <mxGeometry x="485" y="358" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-70" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="1" vertex="1">
          <mxGeometry x="545" y="388" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-71" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="1" vertex="1">
          <mxGeometry x="545" y="358" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-72" value="" style="endArrow=classic;html=1;rounded=0;strokeColor=#B5739D;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="520" y="388" as="sourcePoint" />
            <mxPoint x="540" y="388" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-73" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCE9F;strokeColor=#d79b00;" parent="1" vertex="1">
          <mxGeometry x="485" y="481" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-74" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCE9F;strokeColor=#d79b00;" parent="1" vertex="1">
          <mxGeometry x="485" y="451" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-76" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="1" vertex="1">
          <mxGeometry x="545" y="481" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-77" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="1" vertex="1">
          <mxGeometry x="545" y="451" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-80" value="" style="endArrow=classic;html=1;rounded=0;strokeColor=#CC6600;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="520" y="480" as="sourcePoint" />
            <mxPoint x="540" y="480" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-100" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="638" y="418" width="100" height="100" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-53" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-100" vertex="1">
          <mxGeometry x="70" y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-96" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-100" vertex="1">
          <mxGeometry x="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-97" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-100" vertex="1">
          <mxGeometry x="70" y="30" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-98" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-100" vertex="1">
          <mxGeometry y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-99" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="yMBw17B98Hdd5w8U56Xl-100" vertex="1">
          <mxGeometry x="30" y="70" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-102" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;2. GEMM&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=13;" parent="1" vertex="1">
          <mxGeometry x="626" y="280" width="82" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-105" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFB570;strokeColor=#CC6600;" parent="1" vertex="1">
          <mxGeometry x="790" y="488" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-106" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#CDA2BE;strokeColor=#B5739D;" parent="1" vertex="1">
          <mxGeometry x="790" y="372" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-107" value="&lt;font style=&quot;font-size: 24px;&quot;&gt;$$\oplus$$&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=13;" parent="1" vertex="1">
          <mxGeometry x="770" y="427" width="70" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-108" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;entryX=0.5;entryY=0;entryDx=0;entryDy=0;" parent="1" source="yMBw17B98Hdd5w8U56Xl-106" target="yMBw17B98Hdd5w8U56Xl-107" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="805" y="404" as="sourcePoint" />
            <mxPoint x="805" y="434" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-109" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.5;exitY=0;exitDx=0;exitDy=0;entryX=0.5;entryY=1;entryDx=0;entryDy=0;" parent="1" source="yMBw17B98Hdd5w8U56Xl-105" target="yMBw17B98Hdd5w8U56Xl-107" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="460" y="460" as="sourcePoint" />
            <mxPoint x="510" y="410" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-111" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#FFCCCC;strokeColor=#a31f35;" parent="1" vertex="1">
          <mxGeometry x="849" y="427" width="30" height="30" as="geometry" />
        </mxCell>
        <mxCell id="yMBw17B98Hdd5w8U56Xl-113" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;3. Add&lt;/font&gt;" style="text;strokeColor=none;align=center;fillColor=none;html=1;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=13;" parent="1" vertex="1">
          <mxGeometry x="781" y="338" width="59" height="30" as="geometry" />
        </mxCell>
        <mxCell id="NIhesI-zHesClufHRptb-74" value="" style="shape=flexArrow;endArrow=classic;html=1;rounded=0;endSize=2;startSize=2;endWidth=10.909090909090908;strokeWidth=1;width=8;" edge="1" parent="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="436" y="432.5" as="sourcePoint" />
            <mxPoint x="469" y="432.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NIhesI-zHesClufHRptb-75" value="" style="shape=flexArrow;endArrow=classic;html=1;rounded=0;endSize=2;startSize=2;endWidth=10.909090909090908;strokeWidth=1;width=8;" edge="1" parent="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="591" y="432.5" as="sourcePoint" />
            <mxPoint x="621" y="432.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NIhesI-zHesClufHRptb-76" value="" style="shape=flexArrow;endArrow=classic;html=1;rounded=0;endSize=2;startSize=2;endWidth=10;width=6;" edge="1" parent="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="753" y="386.5" as="sourcePoint" />
            <mxPoint x="777" y="386.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NIhesI-zHesClufHRptb-77" value="" style="shape=flexArrow;endArrow=classic;html=1;rounded=0;endSize=2;startSize=2;endWidth=10;width=6;" edge="1" parent="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="753" y="502.5" as="sourcePoint" />
            <mxPoint x="777" y="502.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NIhesI-zHesClufHRptb-78" value="" style="shape=flexArrow;endArrow=classic;html=1;rounded=0;endSize=2;startSize=2;endWidth=10;width=6;" edge="1" parent="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="819" y="441.5" as="sourcePoint" />
            <mxPoint x="843" y="441.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>

